On the security of modern Single Sign-On Protocols: Second-Order Vulnerabilities in OpenID Connect

OAuth is the new de facto standard for delegating authorization in the web. An important limitation of OAuth is the fact that it was designed for authorization and not for authentication. The usage of OAuth for authentication thus leads to serious vulnerabilities as shown by Zhou et. al. in [44] and Chen et. al. in [9]. OpenID Connect was created on top of OAuth to fill this gap by providing federated identity management and user authentication. OpenID Connect was standardized in February 2014, but leading companies like Google, Microsoft, AOL and PayPal are already using it in their web applications [1], [2], [3], [30]. In this paper we describe the OpenID Connect protocol and provide the first in-depth analysis of one of the key features of OpenID Connect: the Discovery and the Dynamic Registration extensions.We present a new class of attacks on OpenID Connect that belong to the category of second-order vulnerabilities. These attacks consist of two phases: First, the injection payload is stored by the legitimate application. Later on, this payload is used in a security-critical operation. Our new class of attacks - called Malicious Endpoints attacks - exploits the OpenID Connect extensions Discovery and Dynamic Registration. These attacks break user authentication, compromise user privacy, and enable Server Side Request Forgery (SSRF), client-side code injection, and Denial-of-Service (DoS). As a result, the security of the OpenID Connect protocol cannot be guaranteed when these extensions are enabled in their present form. We contacted the authors of the OpenID Connect and OAuth specifications. They acknowledged our Malicious Endpoint attacks and recognized the need to improve the specification [29]. We are currently involved in the discussion regarding the mitigation of the existing issues and an extension to the OAuth specification.

==> sections/aRM.tex <==
\section{\glsfirst{arm}}
\label{sec:arm}

\todo{Ich überlege gerade, ob man es anders strukturieren kann. 1) Was sind BRM und warum sind die gut 2) Was sind aRM und wozu braucht man die. Vorteil: Es werden BRMs gelobt und positiv dargestellt, und aRMs sind eine Erweiterung von gut fundierter Forschung. Nachteil: Wir setzten voraus, dass BRMs etabliert sind. Ich denke das ist nicht so. Vermutlich sind wir die einzigen, die überhaupt wissen, wofür BRM steht. Daher wird das ganze so sehr technisch.}

\Gls{sso} can be described as a sequence of messages transmitted between all three participants. 
A message depicts a request sent from party A to party B and the according response. It is assumed that a message cannot be intercepted and manipulated during the transmission.

In order to analyze a security protocol and execute attacks, the attacker tries to get access to many messages with as less resources as possible. Since the communication between the participants is considered to be secure, the attacker acts in different roles and in this way he gets access to messages.

An \gls{arm} is a message, which is sent or received by the attacker. The attacker can freely choose how to handle this message ,e.g. to manipulate it, to sent a response deviating from the normal protocol flow or just drop it.

Via \gls{arm} the entire \gls{sso} authentication process can be depicted flexible considering an attacker acting with different roles.

\paragraph{Why not \gls{brm}?}
\Glspl{brm} are messages exchanged between \gls{rp} and \gls{op} through the \gls{ua}, e.g. a browser\todo{Ref-BRM}. 
Thus, in order to analyze \glspl{brm} the attacker acts as a normal user navigating his \gls{ua} trough the \gls{sso} authentication. 
However, acting only in one role is a limitation by analyzing \gls{sso} since a limited amount of messages can be analyzed.




\autoref{fig:OIDC_Simple} shows the \gls{oidcp} flow containing nine request and responses. Using the \gls{brm} analyzing model only five messages can be analyzed. The direct communication between Client and OP cannot be considered since the communication occurs directly and not through the \gls{ua}.







==> sections/approachesForAttack.tex <==
\section{Approaches for Attacks}
\label{sec:attackerGolas}

When attacking the \gls{oidcp}, the eventual goal of an attacker is to get unauthorized access to the victim's protected resources.\todo{Stimmt nicht mehr, SSRF, DoS, ... was machen wir hier? Ich würde alles streichen. Wir erkären später einfach was 2nd Order Attacks sind und es sollte reichen...}
There are three main approaches how an attacker can achieve this goal:

\paragraph{Compromise Client Credentials}
In Phase 1 -- during the registration -- the Client receives the \gls{client_id} and the \gls{client_secret}.
Both parameters are used for the Client's authentication to the \gls{op}.
If these credentials are compromised, the attacker can use them to impersonate the Client.

\paragraph{Token Theft}
In \gls{oidc}, there are three different tokens:
The \gls{code}, the \gls{id_token} and the \gls{access_token}.
Leakage of any of them can allow an attacker to get unauthorized access to restricted resources.


\paragraph{ID Token Manipulation}
The \gls{id_token} contains sensitive information about a user's identity.
If the attacker can somehow manipulate the information (fully or partly) contained in it, he may be able to impersonate every user on the \gls{op}.
Note that the \gls{id_token} usually is integrity protected (e.g., by a digital signature), thus, to manipulate it, the attacker has to find a way to circumvent this integrity protection.


==> sections/attackerRoles.tex <==
\section{Attacker roles}
\label{sec:attackerRoles}



==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\begin{table}[H]
	\footnotesize
	\centering
		\begin{tabular}[b]{|p{0.25\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|}
			\hline
			& \bfseries \rotatebox[origin=l]{90}{MITREid Connect} & \bfseries \rotatebox[origin=l]{90}{mod\_auth\_openidc} & \bfseries \rotatebox[origin=l]{90}{\parbox{4.8cm}{Nimbus OAuth 2.0 SDK with\\\centering OpenID Connect extensions}} & \bfseries \rotatebox[origin=l]{90}{\parbox{4.8cm}{Google OAuth Client Library\\\centering for Java}} & \bfseries \rotatebox[origin=l]{90}{Apache Oltu} & \bfseries \rotatebox[origin=l]{90}{phpOIDC} & \bfseries \rotatebox[origin=l]{90}{Drupal OpenID Connect Module~} & \bfseries \rotatebox[origin=l]{90}{pyoidc} & \bfseries \rotatebox[origin=l]{90}{Ruby OpenIDConnect} \\\hline
			\textbf{ID Spoofing} & $\times$ & $\times$ & $\checkmark$ & n/a & n/a & $\checkmark$ & $\times$ & $\times$ & $\times$ \\\hline
			\textbf{Issuer Confusion}	& $\times$ & $\times$ & $\times$ & n/a & n/a & $\times$ & $\times$ & $\times$ & $\times$ \\\hline
			\textbf{\gls{sm}}	& $\times$ & $\times$ & $\times$ & n/a & n/a & $\times$ & $\times$ & $\checkmark$ & $\times$ \\\hline
		\end{tabular}
	\caption[Relying Party Libraries - Applicable Attack-Scenarios]{Relying Party Libraries - Applicable Attack-Scenarios}
	\label{tab:RPAttacks}
\end{table}

\begin{table}[H]
	\footnotesize
	\centering
		\begin{tabular}[b]{|p{0.25\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|p{0.05\linewidth}|}
			\hline
			& \bfseries \rotatebox[origin=l]{90}{Thinktecture IdentityServer v3~} & \bfseries \rotatebox[origin=l]{90}{\parbox{4.8cm}{Nimbus OAuth 2.0 SDK with\\\centering OpenID Connect extensions}} & \bfseries \rotatebox[origin=l]{90}{MITREid Connect} & \bfseries \rotatebox[origin=l]{90}{oxAuth} & \bfseries \rotatebox[origin=l]{90}{Apache Oltu} & \bfseries \rotatebox[origin=l]{90}{phpOIDC} & \bfseries \rotatebox[origin=l]{90}{oauth2-server-php} & \bfseries \rotatebox[origin=l]{90}{pyoidc} & \bfseries \rotatebox[origin=l]{90}{Ruby OpenIDConnect} \\\hline
			\textbf{Sub Claim Spoofing}	& n/a & n/a & $\times$ & $\times$ & n/a & $\times$ & n/a & $\times$ & $\times$ \\\hline
			\textbf{\gls{rum} \#1}	& $\times$ & n/a & $\times$ & $\times$ & n/a & $\times$ & $\times$ & $\times$ &	$\times$ \\\hline
			\textbf{\gls{rum} \#2}	& $\times$ & n/a & $\times$ & $\times$ & n/a & $\times$ & $\times$ & $\times$ &	$\times$ \\\hline
		\end{tabular}
	\caption[OpenID Provider Libraries - Applicable Attack-Scenarios]{OpenID Provider Libraries - Applicable Attack-Scenarios}
	\label{tab:OPAttacks}
\end{table}


==> sections/novelAnalyzingTechniques.tex <==
\section{Second-Order Vulnerabilities in \gls{oidc}}

\subsection{Defining Second-Order \gls{sso} Vulnerabilities}
In this section we explain the class of well-known second-order vulnerabilities in the context of \gls{xss}, \gls{sqlinjection} and \gls{\gls{dos}}. Then, we introduce second-order vulnerabilities in \gls{sso} protocols and reveal novel aspects regarding the security.

In \autoref{fig:webapp2order} is shown an example of classic second-oder vulnerability on an web application.
\begin{figure}[h]
 \centering
 \includegraphics[scale=0.4]{./img/2orderVulnWebApp.pdf}
 %
 \caption{Data flow of a conventional second-order vulnerability on an web application.}
 \label{fig:webapp2order}
\end{figure}

During the first step, the user input containing an attack vector will be stored in the database of an web application. In this step, no attack, but its preparation will be processed.
Later on, the stored attack vector will be pulled from the database and executed leading to an \gls{sqlinjection}, \gls{xss} or even \gls{dos}.

Second-order vulnerabilities in \gls{sso} protocols are more complex since Step 1 and Step 2 of the attack consists of multiple steps and messages exchanged between End-User and Client, Client and \gls{op}, and End-User and \gls{op}.

\begin{figure}[h]
 \centering
 \includegraphics[scale=0.37]{./img/2orderVulnSSO.pdf}
 %
 \caption{test}
 \label{fig:sso2order}
\end{figure}

\autoref{fig:sso2order} shows the data flow within a second-order vulnerability in a \gls{sso} protocol.
Similar to Step 1 in classic second-oder attacks, the attacker stores the attacks vector. The main difference is that the user input $\alpha$ is not the attack vector. $\alpha$ justs starts the \gls{sso} authentication.
The injection of the attack vectors occurs during \emph{Phase 1} of the protocol -- the Discovery phase within a Server-to-Server communication. The attacker returns data used later on during the protocol. 
In case of \gls{oidc} this is a metadata file containing endpoints of the \gls{op}, supported protocol flows and supported cryptographic algorithms.

In Step 2 the stored attack vectors will be loaded and used during the different phases of the protocol. In dependence 

We first need to define a \emph{second-order vulnerability} in \gls{sso}.
Common second-order vulnerabilities in web applications as shown in~\cite{Dahse2014,Olivo2015} have only three entities involved:
\begin{inparaenum}
	\item the attacker acting with his browser,
	\item the server hosting the web application and
	\item optionally another End-User (the victim).
\end{inparaenum}
In case of \gls{\gls{dos}} attacks as shown in~\cite{Olivo2015}, there is no third entity involved, since the victim is the server hosting the web application itself.

Due to the nature of \gls{sso}, we have more entities:
\begin{inparaenum}
	\item the End-User who wants to login. This can be either a benign End-User or the attacker.
	\item the \glsfirst{sp} which is the main target of our attacks.
	\item a honest \glsfirst{idp}.
	\item an attacker who can host his own web application on the Internet. We will use this server to host a malicious discovery service later on.
\end{inparaenum}

To summarize, in the classical web application scenario, we have one attacker entity and two benign entities, while in the \gls{sso} scenario, we have one more benign entity.

\begin{definition}[Second-order \gls{sso} Vulnerability on an \gls{sp}]
	Let $U$ be an End-User, let $S$ be an \gls{sp}, let $I$ be a honest \gls{idp} and let $A$ be the attacker.
	We say that $S$ contains a second-order \gls{sso} vulnerability, if:
	\begin{enumerate}
		\item $A$ can place a harmless\footnote{\emph{Harmless in this context means, that the payload is not directly executed and as such, it does not influence $S$ in any kind.}} payload on $S$ in such a a way that
		\item the further communication process between $S$, $i$ and $U$ is
		\begin{enumerate}
			\item either slowed down significantly due to a \gls{\gls{dos}} attack or
			\item $A$ gets access to resources owned by $U$.
		\end{enumerate} 
	\end{enumerate}
\end{definition}

As explained in this definition, the attacker does not start the payload execution itself.
He just places it on the \gls{sp}.
The execution of the payload takes places in the further protocol flow, for example, if the End-User enforces the \gls{sp} to load the payload in order to continue the \gls{sso} protocol.

\todo{Definition überarbeiten!}

\subsection{\gls{oidc}: Dynamic Client Registration}

The information flow during the automated client registration is shown in \autoref{fig:OIDC_DynReg}.
Initially, the End-User submits his \emph{identity}, for example \emph{alice@honestOP.com}, to the Client.
In order to initiate the \gls{sso} authentication, the Client needs to discover the corresponding \gls{op} controlling the identity of Alice.
Thus, in Phase 1.1, the Client uses the provided \emph{identity} and extracts the domain name of the \gls{op}~\cite[Section 2.1]{OpenIDFoundation2014a}.
In our example, Alice's identity is controlled by the domain \emph{honestop.com}.
The domain name uniquely identifies the corresponding Discovery endpoint\footnote{This is usually realized by applying a modifier to the domain, e.g., \texttt{https://honestop.com/}\emph{.well-known/webfinger}.}.

The Client sends an HTTP request to this Discovery endpoint and subsequently retrieves the \gls{op}'s configuration information including its endpoint locations:
The (Dynamic) Registration Endpoint (\emph{regEndp}), the Authorization Endpoint (\emph{authEndp}), the Token Endpoint (\emph{tokenEndp}) and further endpoints (c.f., \autoref{sec:basics:endpoints}).

In Phase 1.2 (Dynamic Registration) the Client can automatically register on the \gls{op}.
For that purpose, the Client sends its own URL, for example \texttt{http://client.com}, to the \emph{regEndp} URL.
The \gls{op} responds with a \gls{client_id}/ \gls{client_secret} pair.
Finally, the Client and the \gls{op} store the credentials in their respective databases and use them during the next phases.

\subsection{How does the Discovery phase influence the \gls{oidc} flow?}

By analyzing the Discovery and Dynamic Registration phases we make the following observations:

\begin{itemize}
    \item The usage of custom \glspl{op} is supported by the \gls{oidcp} without any pre-configuration, installation or manual interaction (neither on the Client nor on the  User-Agent).
    The End-User has to enter his identity on the Client, e.g. \texttt{bob@honestOP.com}, in order to start the authentication with his custom \gls{op}.

    \item All discovered endpoints are URLs.
    There are no limitations specified that restrict these URLs to domains, subdomains, or URL contexts.
\end{itemize}

Based on our observations, we realized that we can trigger any Client supporting Discovery and Dynamic Registration to use our custom \gls{op} for authentication.
Thus, we control the data sent to the Client and used in the next phases of the protocol flow. In \autoref{fig:metadataInfluence} we present how the retrieved information during the Discovery phase influences the \gls{oidc} phases.
\begin{figure}[!ht]
 \centering
 \includegraphics[width=\linewidth]{./img/OIDC_Metadatainfluence.pdf}
 %
 \caption{A detailed overview of the Discovery phase revealing how the metadata received by the Client influences the next OpenID Connect phases.}
 \label{fig:metadataInfluence}
\end{figure}

The first two messages are used to discover the URL where the metadata of the \gls{op} is stored based on the identity entered by and End-User. The \emph{Discovery request -- 1.1.1} is an HTTP message sent to the \gls{op}'s discovery service (e.g.\emph{ \url{https://honestOP.com/.well-known/webfinger}}). The response is a JSON message containing two parameters: 
\begin{inparaenum}
	\item \emph{href}, which points to the metadata of the \gls{op} and 
	\item \gls{rel}, which identifies the type of service (e.g. \emph{\url{http://openid.net/specs/connect/1.0/issuer}}).
\end{inparaenum}

Consequentially, a new HTTP request is sent to the URL specified via the \emph{href} parameter. The response contains the metadata with all information regarding the \gls{op}: endpoints, supported authentication flows, supported algorithms for signing and encrypting messages, public keys of the \gls{op} etc.

\autoref{fig:metadataInfluence} depicts the relation between the endpoints received in the last messages of the Discovery phase and the \gls{oidc} phases.
The \emph{regEndp} will be used by the Client in order to register the Client on the \gls{op} and receive the client credentials (e.g. \emph{client\_id/client\_secret}).

The \emph{authEndp} points to the Authorization server responsible for the authentication of the End-User. Noteworthy is the fact, that only the Authorization server is visible for the End-User during the authentication. All other endpoints are called by the Client directly and thus cannot be seen by the End-User.

The next three endpoints \emph{tokenEndp}, \emph{userInfoEndp} and \emph{jwksEndp} are used in the last Phase (Phase 3) of the protocol: the End-User authentication. 

\subsection{Security consideration regarding second-order vulnerabilities}
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%


\gls{oidc} supports the usage of custom \glspl{op}.
%
For that purpose, a Client uses the Discovery and the Dynamic Registration Phase to retrieve the \gls{op}'s configuration information including the endpoints \emph{regEndp}, \emph{authEndp}, \emph{tokenEndp}/\emph{userInfoEndp}/\emph{jwksEndp} and registers on it. 

Please note that a malicious Discovery service can freely choose all these parameters (cf., Phase 1.1 in \autoref{fig:OIDC_DynReg}).
By this means, the malicious Discovery service can influence 
\begin{inparaenum}
	\item which URL the Client registers (\emph{regEndp}),
	\item which URL is used by the End-User to authenticate (\emph{authEndp}),
	\item and to which URL the token will be finally sent (\emph{tokenEndp/userInfoEndp}).
\end{inparaenum}

%
%

%

%
%
%


%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%


==> sections/otherAttacks.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

==> sections/tainting.tex <==
\section{Tainting Checking}
\label{sec:tanting}

Tainting is a concept to specify parameters, which cannot be considered as trusted and has to be verified before being consumed. 

Tainting is used usually on context of attacks like SQL injection and buffer overflow attacks. However, we adapted this concept on \gls{sso} and as a result we found novel attacks on the \gls{oidcp}. 


\subsection{Tainting the Dynamic Registration}

\subsection{Tainting the Redirects}

\subsection{Tainting the ID Token}

\subsection{Tainting the Access Token}

==> stuff/lstlistingstyles.tex <==
\newcommand\JSONnumbervaluestyle{\color{blue}}
\newcommand\JSONstringvaluestyle{\color{red}}

%
\newif\ifcolonfoundonthisline

\makeatletter

\lstdefinestyle{json}
{
  showstringspaces    = false,
  keywords            = {false,true},
  alsoletter          = 0123456789.,
  morestring          = [s]{"}{"},
  stringstyle         = \ifcolonfoundonthisline\JSONstringvaluestyle\fi,
  MoreSelectCharTable =%
    \lst@DefSaveDef{`:}\colon@json{\processColon@json},
  basicstyle          = \ttfamily\scriptsize,
  keywordstyle        = \ttfamily\bfseries,
  captionpos=b, %
  breaklines=true, %
  frame=shadowbox, %
  numbers=left,
  xleftmargin=1.5em,
  xrightmargin=1.1em,
}

%
\newcommand\processColon@json{%
  \colon@json%
  \ifnum\lst@mode=\lst@Pmode%
    \global\colonfoundonthislinetrue%
  \fi
}

\lst@AddToHook{Output}{%
  \ifcolonfoundonthisline%
    \ifnum\lst@mode=\lst@Pmode%
      \def\lst@thestyle{\JSONnumbervaluestyle}%
    \fi
  \fi
  %
  \lsthk@DetectKeywords%
}

%
\lst@AddToHook{EOL}%
  {\global\colonfoundonthislinefalse}

\makeatother
